Sunstar: A Cost-effective Multi-Server Solution for Reliable Video Delivery

In spite of much progress and many advances, cost-effective, high-quality video delivery over the internet remains elusive. To address this ongoing challenge, we propose Sunstar, a solution that leverages simultaneous downloads from multiple servers to preserve video quality. The novelty in Sunstar is not so much in its use of multiple servers but in the design of a schedule that balances improvements in video quality against increases in (peering) costs. The paper's main contributions are in elucidating the impact on the cost of various approaches towards improving video quality, including the use of multiple servers, and incorporating this understanding into the design of a scheduler capable of realizing an efficient trade-off. Our results show that Sunstar's scheduling algorithm can significantly improve performance (up to 50% in some instances) without cost impacts.

==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#
# $Id: 
#

.SUFFIXES:
.SUFFIXES: .ps .dvi .tex

TEXINPUTS := .:${TEXINPUTS}
BIBINPUTS := .:${TEXINPUTS}

#all: eps dvi ps pdf # res
all: pdf
eps: fig obj

#PAPER=mosaic
PAPER=main

LATEX=pdflatex

ps:  $(PAPER).ps

pdf: $(PAPER).pdf
dvi: $(PAPER).dvi

obj: $(patsubst %.obj, %.eps, $(wildcard *.obj))
fig: $(patsubst %.fig, %.eps, $(wildcard *.fig))

res:
	make -C results
	make -C figs

clean:
	$(RM) *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx *.out *.bak
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

distclean: clean
	$(RM) $(patsubst %.fig, %.eps, $(wildcard *.fig))
	$(RM) $(patsubst %.obj, %.eps, $(wildcard *.obj))

# only need -Ppdf if using CM fonts
#%.pdf: %.dvi $(wildcard *.bib)
#	dvips -Ppdf -G0 -t letter -o $*.tmp.ps $<
#	ps2pdf $*.tmp.ps $*.pdf
#	$(RM) $*.tmp.ps $*.dvi *.aux *.log *.bbl *.blg *.toc

%.pdf: $(wildcard *.tex) $(wildcard *.bib)
	$(LATEX) $*
	bibtex $*
	$(LATEX) $*
	if [ -e $*.toc ] ; then $(LATEX) $* ; fi
	if [ -e $*.bbl ] ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	#dvips -t letter -z -Ppdf -G0 -D600 main.dvi -o main.ps
	#ps2pdf main.ps main.pdf

	$(RM) *.aux *.log *.bbl *.blg *.toc

%.ps: %.dvi
	dvips -Ppdf -G0 -tletter -o $@ $<
%.ps.gz: %.ps
	gzip -v9 $<

%.eps: %.obj
	tgif -print -eps $*

%.eps: %.fig
	fig2dev -L eps $< $@


==> intro_RG.tex <==
\section{Background and Motivations}
\label{sec:intro}

The growing importance of video traffic on today's network
infrastructure is by now well-documented. The share of video traffic
on North American networks exceeded $70\%$ of peak hour traffic in
early 2016 and is expected to surpass $80\%$ by the end of
2020~\cite{sandvine16}. In other words, video is by far the dominant
traffic contributor on fixed network links, and while its
contributions to mobile access links is slightly lower (about $40\%$),
it remains a major factor there as well.  This increasing dominance is
in spite of continued progress in encoding efficiency, \eg x265 or VP9
codecs~\cite{kufa15,uhrina14,ozer16}, and has played a major role in
persistent problems when it comes to ensuring quality video delivery.
For example, Conviva VXR reports, \eg\cite{vxr14,vxr15,conviva15},
which each year track various video performance metrics, report that
buffering events (periods during the video stalls to replenish its
playback buffer) remain common (from $20\%$ to $40\%$ depending on
location), as do drop in video resolution while playing (those affect
over $50\%$ of all videos). Equally important, degradation in video
quality is also known to have a major impact on users' behavior and their
satisfaction with Internet video~\cite{krishnan12}.  This is obviously
of concern, as has been articulated in several recent industry forums
focused on video
delivery~\cite{cdnsummit13,cdnsummit14,cdnsummit15,cdnsummit16}.

A first goal of this paper is, therefore, to explore possible
solutions to remedy this situation and improve the quality of Internet
video delivery.  Of interest in this context is the use of multipath
solutions, and in particular solutions that let video clients download
video segments (chunks) simultaneously from multiple servers.
We refer to such solutions as {\em Multipath-MultiServer (MuMS)},
\eg\cite{dynamic,youtuber}.
Reliance on multiple paths from distinct servers can help mitigate
exposure to quality degradations caused by network congestion, failure
of individual paths, and server overload.  In particular, multipath
has been shown to be useful in improving throughput and reliability in
both wired and wireless
networks~\cite{apostolopoulos04,Chen:2004ih,chen09,ganesan2001highly,golubchik02,Radi:2012en},
and there is initial evidence that it could also benefit
delay~\cite{javed09} as well as rate stability~\cite{arzani12}.  The
latter is of particular interest, as rate variations are a major
factor in video quality degradation.

Specifically, a typical video streaming client operates in two
phases~\cite{rao11}: pre-buffering and re-buffering.  A video is split
into segments (chunks), and in the pre-buffering phase the client
requests chunks at the maximum rate allowed by the
network\footnote{This holds for both video download and
  live-streaming, though with obvious limitations on the pre-buffering
  phase for the latter.}. Once the client deems there are enough
chunks in its playback buffer, it starts playing the video and
switches to re-buffering mode. In this mode, the client requests
chunks at a fixed rate determined by the encoding rate.  Video
playback proceeds smoothly as long as chunks are available in the
playback buffer before they need to be payed-out.  Variations in the
available transmission capacity between the server(s) and the client
can result in late delivery or loss of video chunks.  This in turn
depletes the playback buffer and can eventually induce video stalls or
skips.  Minimizing variations in the transmission rate at which the
clients can download chunks, if feasible, should therefore limit
fluctuations in the playback buffer content and consequently minimize
instances of stalls or skips.  Exploring how to best achieve such a
goal across a wide range of configurations, including different types
of video streams and codecs, is one of the goals of this proposal.

Another goal of the paper is to realize these improvements, while
at the same time mitigating any impact they may on the peering costs
of video providers, \ie the costs they incur from Internet Service
Providers (ISPs) for delivering video to their customers.  Ensuring
that better quality in video delivery does not translate into higher
peering costs is of particular importance given the low profit margins
under which most video providers operate~\cite{ball15,bonte10,cox13}.
Of concern in our context is the extent to which reliance on multiple
paths can indeed result in higher peering costs.  The possibility of
such increases is in hindsight relatively intuitive.  In particular,
most ISPs use a 
charging model that lies in between charging for average usage and
peak usage, \eg by charging based on the $95^{\mbox{th}}$ percentile
computed for usage during $5$~mins intervals over a period of a
month\footnote{See
  \url{https://www.noction.com/blog/95th_percentile_explained.}}.
Spreading transmissions over multiple paths can increase the odds of a
higher overall $95^{\mbox{th}}$ percentile cost, \ie assuming a total
traffic that is split over two paths in proportions $x_1$ and $x_2$,
we typically have:  $95^{\mbox{th}}\mbox{ percentile of } (x) =
95^{\mbox{th}}\mbox{ percentile of } (x_1+x_2) \leq
95^{\mbox{th}}\mbox{ percentile of } (x_1)+95^{\mbox{th}}\mbox{
  percentile of } (x_2)$. As a result, exploring mechanisms 
that can limit any such increase while preserving the benefits of a
multi-path solution when it comes to video quality is of interest.

\emph{RG:  Need to add paper's contributions and paragraph outlining
  the rest of the paper's structure.}


==> overview.tex <==
\section{\Sys Client Design}
\label{sec:design}

As discussed in Section~\ref{sec:mums}, realizing the lowest possible
cost calls for downloading at the lowest possible rate, while meeting
the video's target rate of~$T$.  Blindly following such a
recommendation is, however, likely to result in poor performance.
\Sys seeks to instead minimize rate \emph{variance}, while
guaranteeing a sufficient average download rate.  Minimizing rate
variance still favors lower rates, but at the same time also aims for
rate stability.  A more stable download rate can, in turn, mitigate
playback disruptions by ensuring a regular replenishing of the
playback buffer, even during periods of network fluctuations.

%% Based on earlier results, an optimum client design \textit{should}
%% be one which guarantees an acceptable download rate at the smallest
%% possible variation. This means that the client should aim to
%% download at the minimum possible rate that is sufficient to ensure
%% that it never stalls. It should also ensure that the variations
%% around this rate are small so as to cause minimal disruption to
%% playback whenever network conditions change abruptly.

%% This not only improves clients performance as it reduces the need
%% for changes in bit rate, but also should result in the smallest
%% possible impact on cost.  In the rest of this section, we present
%% the design and implementation of \Sys that aims to achieve the
%% above two goals.

\Subsection{\Sys Client Design Overview}

The \Sys client design assumes that video content is replicated across
multiple servers. Upon requesting a video, a client is assigned a
given set of servers. This is done through a server selection
algorithm imposed by the provider and can be realized through manifest
files that clients can download from a designated server. The client
is an application layer client that downloads and plays back videos by
sending requests for fixed size chunks to its assigned servers using
{\tt http range} requests. It adapts the number of chunks requested
from each server at runtime based on current performance measures.
This calls for both estimating the bandwidth available to each server
to avoid congesting the network or servers, and for distributing
requests across paths to meet cost and performance objectives. Note, that an alternative to 
an approach that estimates the number of requests sent to each server (for fixed sized chunks) would be one such as that of~\cite{youtuber} that
estimates the size of each request. This approach, however, is ineffective in the face of link variations as 
its reaction time is limited by the size of each chunk (see \S\ref{sec:eval}), i.e. the client needs to wait for responses from the servers to send the next request.

The current \Sys client has the following capabilities:

\noindent {\bf Bandwidth estimation.} It is important that the SunStar client utilizes the available bandwidth effectively
and does not exacerbate congestion if/when it happens. Thus, in our design of the SunStar client, we maintain an estimate
of the bandwidth available on each path using a TCP-like
mechanism, which computes a window size (in chunks) for each path.
This provides upper bounds for the number of requests that can be sent
to each server. Specifically,
we use a TCP CUBIC congestion control mechanism to adapt the window
size to server~$i$. We pick CUBIC as our bandwidth estimation method as the congestion window changes are solely dependent on the time of the last congestion event
and not the latency to the server (this is important as we use multiple servers in the client and there might be large discrepancies in the RTT to each of these servers).
Note that CUBIC relies on losses to reduce
its window size, and since chunks are requested over {\tt http},
there is no application level loss in the \Sys client. We
use a drop of more than $20\%$ in the estimated average rate to
server~$i$ as equivalent to a CUBIC packet loss. This average rate is estimated using an 
exponential average (as it acts as a low pass filter and eliminates estimation noise) of request completion times.

\begin{figure*}[hbtp!]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
   \includegraphics[width=.8\linewidth]{Figures/SinglePath-BufferEmptyTime.png}
\vspace{-1mm}
     \caption{Distribution of the fraction of time clients stalled in each run. \label{fig:stallsSinglePath}}
\vspace{-1mm}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
\includegraphics[width=.8\linewidth]{Figures/SinglePath-Comparison-chunksSkipped.png}
\vspace{-1mm}
     \caption{Distribution of the number of chunks skipped in each run. \label{fig:skippedSinglePath}}
\vspace{-1mm}
\end{subfigure}
\vspace{-1mm}
\caption{Comparison to single server. {\bf High} and {\bf Medium}
  $C_i$, smooth bandwidth variations.} 
\vspace{-1mm}
\end{figure*}


\noindent {\bf Request scheduling.} The client dynamically adapts the
number of chunks to request from each server. The \Sys scheduler
(Section~\ref{sec:scheduler}) aims to optimize the user's QoE by
allocating chunk requests to minimize rate variability.

\noindent {\bf Out-of-order delivery.} As with other multipath
solutions, chunks requested from different servers may arrive out of
order. We take an approach similar to MPTCP in dealing with this
issue, namely, split the client design into two layers. The lower layer
consists of individual {\tt http} connections or {\em subflows}, each
responsible for sending requests to a single server. Upon receiving
responses to requests, the subflow passes them up to the upper layer
that reassembles them in the correct order.

%This should
%  be done so as to optimize the user's QoE and is the job of the MuMS
%  scheduler. The scheduler, using rate estimates to each server,
%  allocates chunk requests to each subflow. We describe its design in
%  Section~\ref{sec:scheduler}.

\noindent {\bf Performance optimizations.} The \Sys client
incorporates optimizations previously devised for MPTCP. In
particular, it employs opportunistic retransmit. When latencies across
servers are significantly different, opportunistic retransmit prevents
the client from stalling while waiting for a chunk requested from a
high latency server.  A mechanism similar to TCP time-outs is also
implemented for chunk requests. If a response is not received before a
time-out, the request is re-sent to another server.  Last, we limit the
number of retries for chunk requests to bound playback stalls.  Once
this retry limit is exhausted, the chunk is skipped and the player
relies on its codec to mask missing frames.
%% This is to minimize the number of playback stalls.

We acknowledge that an alternative to an application layer solution is
a transport layer one, \ie by extending a protocol such as MPTCP. A
transport layer solution has advantages such as finer adaptation
granularity and, therefore, faster reactions. However, extending MPTCP
to work in a multi-server rather than single-server setting involves
non-trivial changes to the network protocol stack.  In addition, the
tight coupling of MPTCP components can result in unexpected
interactions~\cite{arzani14}.  Avoiding or predicting them calls for a
careful evaluation of proposed changes. Hence, an application layer
solution offers a number of benefits, in terms of flexibility and ease
of deployment.

Note also that while, as mentioned earlier, \Sys is complementary to
ABR solutions, combining \Sys with an effective ABR strategy, \ie
deciding when to adjust coding rates, is not addressed in the current
\Sys client design.  Extending the design to make it fully compatible
with ABR solutions is part of future work.

%\vspace{-1mm}
\subsection{The \Sys Scheduler}
\label{sec:scheduler}

%As mentioned earlier, 
The scheduler is the core component of the \Sys client\footnote{We
  show in Sections~\ref{sec:eval} and~\ref{sec:cost} that it not only
  delivers significantly better performance than other schedulers, but
  that it realizes those performance improvements with little to no
  impact on cost.}. Its main goal is to minimize playback stalls (and
therefore skips) as
their frequency and duration are known to have a significant influence
on users' QoE~\cite{QoE1,QoE2} (see also our Mechanical Turk
experiments in Appendix~\ref{appendix:turk}).  Playback stalls are a
direct consequence of an empty playback buffer, which arises when the
download rate falls below the playback rate for an extended period of
time. To minimize the odds of such occurrences, the \Sys scheduler
periodically runs an optimization that computes how many
chunks to request from each server to ensure a target average download
rate while minimizing variations around that average rate. Note, that our design is informed by
the findings of Theorem~\ref{theo:cost}. Namely, \textit{we choose our target rate as the lowest acceptable value in order
to minimize the multipath client's impact on cost. We minimize variations around that rate in order to prevent performance degradations in the face of congestion and/or link variations.}

The optimization is greedy and myopic, \ie based on current
performance estimates for the paths to each server and does not
attempt to predict future performance. It operates in
``epochs'' or ``rounds'', whereby in each epoch it seeks to minimize
the \textit{increase} in variance in that round.  The optimization
takes as input the current window size of each server (an upper bound
on its rate), its current estimate of the (average) rate to each server, and
the number of pending requests to each server.  It then computes a
target rate (number of requests) for each server in the next epoch.
This rate is used by the scheduler to schedule requests to
the servers.

%% The (adaptive) window size that is used as input to the optimization
%% helps avoid overwhelming any one link/server and is an upper bound on
%% the rate a client can request chunks from a given server.
The rest of this subsection describes the formulation of this
optimization process in more details.

\subsubsection{Scheduler Optimization}
\label{sec:sched_optim}

%at the start of each round aims to minimize the increase
%in variance in that round. 
%% Our MuMS scheduler aims to greedily minimize the worst case
%% increase in running rate variance while ensuring that the running
%% mean is larger than a nominal value. 

Let $\mathcal{S}$ be the set of servers assigned to a MuMS
client. The goal is to guarantee each client an average
rate~$T$ (this value can be specified by ABR), while minimizing \textit{changes} in the running variance:
%\vspace{-1mm}
\begin{align}
(\sum_{i\in \mathcal{S}}{\alpha_{i} R_i} - T)^2,
\end{align}
where $R_i$ is the inverse of the time it takes for requests to arrive
from server $i$ (in other words $R_i$ is the inverse of the application
level round trip time), and $\alpha_i$ is the number of
chunks that the client should request from server $i$. The client's
attained rate is thus $\sum_i\alpha_i R_i$. 

This translates to solving the following optimization:
%\vspace{-1mm}
\begin{align}
\label{eq:opt1}
&\min_{\alpha} \mid \sum_{i \in \mathcal{S}} \alpha_i R_i - T \mid\\
&s.t. \quad  \sum_{i \in \mathcal{S}} \alpha_i \widehat{R}_i \ge T \nonumber\\
&\quad \quad \quad \alpha_i \le w_i \nonumber,
&\end{align}
%
where $\widehat{R}_i$ is the expectation of $R_i$, and $w_i$
the current (CUBIC) window size\footnote{Note, that this window size serves as an upper bound on the number of requests that can be sent to each server.} to server $i$. The $\alpha_i$ are the decision variables in this formulation and determine the number of requests allocated to each server. Let $R_i^u$ and
$R_i^l$ be upper and lower bounds for $R_i$, respectively.  $R^u$ and
$R^l$ can be estimated using Chebychev's inequality by identifying the upper/lower bounds on the $95$ and $5$ percentiles of the distribution of $R$.
\Eqref{eq:opt1} is then equivalent to:
%\vspace{-3mm}
\begin{align}
\label{scheduler}
&\min_{\alpha,t} \quad t  \\
&s.t. \quad \sum_{i \in \mathcal{S}} \alpha_i \widehat{R}_i \ge T \nonumber\\
&\quad \quad \sum_{i \in \mathcal{S}} \alpha_i \widehat{R}^u_i \le T+t \nonumber\\
 &\quad \quad \sum_{i \in \mathcal{S}} \alpha_i \widehat{R}^l_i \le T-t \nonumber\\
&\quad \quad \alpha_{i} \le w_i \nonumber.
\end{align}
%
\Eqref{scheduler} is derived
by first converting the absolute value form of the problem to its
linear form and then replacing the two resulting bounded constraints
with tighter bounds through $R_i^u$ and $R_i^l$.

The above formulation assumes integer values for $\alpha_i$, but
this can occasionally result in significant overshoots in the realized
rate.  We, therefore, use fractional values for $\alpha_i$.
%% and instead use $\alpha_i R_i$ as the rate of request to server $i$
%% within an epoch. 
Because requests are for an integer number of chunks, we
maintain a state variable that accounts for the ``excess'' rate $y_i$
to each server.  After solving the optimization, we compute
$\max(\alpha_iR_i-y_i,0)$ and use this value as the target rate to
server~$i$. When this corresponds to a fractional number of chunks, we
then round it up and update $y_i$ accordingly.
%% Once we have made up for any ``excess'' bandwidth we reset the
%% value to~$0$. 

There are two other aspects to the above optimization that need
discussion, as they affect the implementation of the \Sys scheduler.

%% \vspace{1mm}
The first is \emph{Dealing with Infeasibility.} As network bandwidth 
fluctuates, the optimization may not always be
feasible. However, we still want the client to request the best
possible transmission rate. For that purpose, we progressively
decrease the target rate~$T$ (by~$10\%$ in our experiments) and rerun
the optimization until a feasible solution is found.  Conversely,
following a period of rate deficit, we seek to increase the target
rate whenever feasible to make up for the deficit.  Specifically, we
run the optimization for a higher target rate (typically~$30\%$) until
the deficit has been absorbed.
%% , $T$ is multiplied by a value $\beta$ where $\beta \ge 1$ (we use
%% $\beta=1.3$). Again, we continue this multiplication until we reach
%% the original value of $T$. We bound $T$ to never go above the
%% original specification of the user or below half of that
%% specification, i.e. if we use $T'$ as the user's original
%% specification for $T$, then $T \in [ \frac{T'}{2},T']$.
%%

%\subsection{Breaking Ties}

%\vspace{1mm}
The second issue concerns \emph{Breaking ties.} The optimization needs
not have a unique solution, \eg with homogeneous paths with sufficient
bandwidth, using any of them is a feasible and optimal solution. We,
therefore, add two tie-breaking criteria to the optimization: (1) we
minimize the number of servers used, and (2) we favor those that have
been used more frequently in the past. Both criteria aim to reduce the
number of out-of-order chunks.



We show in Section~\ref{sec:exec} that the optimization of
\Eqref{scheduler} is practical in that it can be solved for up to $4$
servers in around $1$ms without overloading an entry-level
machine.
%%\footnote{Note though, that the complexity of solving the problem
%%grows relatively fast with the number of servers and variables.}. 
We also note that it is possible to improve the
optimization run time by re-using past solutions as a starting point
in each round~\cite{bertsimas}.  
%Finally, further optimizations are also possible
%\textcolor{red}{[RG: WE MAY WANT TO BE A BIT MORE SPECIFIC HERE]} that
%would allow the optimization to run on low-end devices, \eg cell
%phones. 
%BA: I had zero context as to what that sentence was referring to, and I have no idea if it is possible at all which is why I removed the whole thing.
Such improvements are, however, beyond the scope of this
paper.

%% In Section~\ref{sec:eval} we evaluate the performance of the \Sys's
%% scheduler and show that it significantly outperforms a basic
%% scheduler based on selecting servers with the lowest RTT. In
%% addition, we show in Section~\ref{sec:cost} that it is also
%% successful in Our schedule reduces cost for providers compared with
%% other schedulers.


==> scratch <==






\eat{
A \Sys clients assumes that video content is replicated across
multiple servers. Upon requesting a video, the client is assigned a
given set of servers. This is done through a server selection
algorithm imposed by the provider and can be realized through manifest
files that clients can download from a designated server.  The crux of
the \Sys design is, however, in how the client schedules transmission
requests across its assigned servers so as to realize the best
possible trade-off between cost and performance (video quality).

%% The \Sys client, aims to ensure high video quality while keeping
%% the content provider's cost as low as possible. 
The investigation of \S\ref{sec:trade-off} showed that minimizing
costs calls for downloading videos at the lowest rate possible ($T$).
However, barring an unacceptably long pre-buffering phase (to build-up
the playback buffer), blindly downloading at $T$ will result in poor
performance, as it makes the playback buffer vulnerable to lulls
(below $T$) in network bandwidth.  Such lulls are unavoidable in the
Internet, and the challenge is then in compensating for them with
rate increases that are as low as possible while still avoiding
instances of buffer underflow.  To address this challenge, \Sys's
scheduler introduces a formal metric to quantify this trade-off, and
uses it to determine how to adapt its download rate from each server.

%% to meet a target average rate guarantee, goal is in guaranteeing a
%% low download rate $T$, while ensuring that clients performance is
%% not impacted by variations in network conditions (given that $T$ is
%% low and might not provide sufficient buffering to ``ride out'' such
%% variations).

%% Network variations typically translate to variations in the rate of
%% download from each server.  As shown in \S\ref{sec:why_cost}, such
%% rate variations (in the long term) not only impact performance but
%% also results in higher costs in a multipath scenario (refer to the
%% discussion on the convexity of the max function).
Specifically, after a short initial pre-buffering phase intended to
``prime'' its playback buffer, \Sys seeks to schedule transmissions
across paths so as to minimize rate variations around the target rate
of $T$.  More formally, \Sys's objective is to minimize rate
\emph{variance}, while guaranteeing an average download rate equal to
the video's long term average (denoted as $T$). Once again, here, $T$ is the lowest acceptable (average) rate that
the video player can tolerate without experiencing performance degradations.

There are a number of metrics that can be used in order to quantify performance. These include 
buffer size variations and/or the frequency/probability of experiencing an empty buffer scenario. However, 
by minimizing variations around the playback rate $T$ we argue that we can also indirectly control changes in 
these metrics as well. To illustrate this, take $T$ as the playback rate of the client and $R$ as the instantaneous download rate
of the client. The client's playback buffer size therefore changes in direct proportion to $R-T$, where $R-T < 0$ indicates a depletion in
playback buffer content (or potentially an empty playback buffer). Given that we assume a constant value for $T$, by minimizing the long term variations in $R$
we also reduce long term variations in playback buffer size. By ensuring that the average R is larger than T and minimizing its variance we also indirectly can reduce the frequency 
of an empty playback buffer (see~\S\ref{sec:eval}). From a cost standpoint, this has the advantage of targeting the
minimum overall possible rate, while keeping increases above it as low
as possible.  

The client is an {\em{application}} that downloads and plays back
videos by sending requests for chunks (video segments) to its assigned
servers using {\tt http range} requests.
Turning next to the overall software architecture of the \Sys client, \fig{fig:architecture} offers an
overview of its main building blocks.

  
 


\Sys requires a number of building blocks in
order to estimate network characteristics on path to each server (to
decide the number of requests it needs to send) as well as a means of
deciding how many requests to send to each server at each point in
time. 
}

%In the rest of this section, we will describe each one of these building blocks in greater detail.

%These operations form the core building blocks of \Sys as
%follows:

%We summarize the three main components below:

%\noindent{\textbf{The \Sys Scheduler (\S\ref{sec:scheduler})}}: 


%This is partially due to the fact that by using fixed sized chunks we can estimate the typical arrival time of requests from each server and use this estimate in order to re-send requests when a response is deemed ''late''. Doing so for variable sized chunks is more difficult. This is because we are estimating the delivery time of HTTP chunks, the size of the chunk impacts TCP e.g., time spent with a zero receive window, and therefore linearly scaling the estimated delivery time based on the chunk size is not an option.
%This is because the second
%approach (that of~\cite{youtuber}) is ineffective in the face of link
%variations given that its reaction time is limited by the size of each
%chunk (See~\S\ref{sec:eval}) \ie, the client needs to wait for
%responses from the servers to send the next request (each chunk request is designed to utilize the full available bandwidth from each server).
%\Sys adapts the number of chunks requested from each server based on
%current performance measures. This is achieved through the \Sys
%scheduler. 



%Other core functionalities provided by
%the request manager are described in \S\ref{sec:manager}.
{\eat
\noindent{\textbf{Bandwidth Estimator (\S\ref{sec:core})}}: To
identify the number of requests that the client should send to
servers, the scheduler requires (as input) estimates of the bandwidth
available to each of them. This is the job of the bandwidth estimator
to maintain a running estimate of the current bandwidth to each server
by tracking the corresponding response times.

\noindent{\textbf{Request Manager (\S\ref{sec:manager})}}: Once the
scheduler determines the number of requests to be sent to each server,
it inputs that information to a request manager. The request manager
ensures not only that the appropriate number of requests are sent to
each server, but also that the responses are placed in the playback
buffer in the correct order. 
}
